A Theoretical Perspective on Differentially Private Federated Multi-task Learning

In the era of big data, the need to expand the amount of data through data sharing to improve model performance has become increasingly compelling. As a result, effective collaborative learning models need to be developed with respect to both privacy and utility concerns. In this work, we propose a new federated multi-task learning method for effective parameter transfer with differential privacy to protect gradients at the client level. Specifically, the lower layers of the networks are shared across all clients to capture transferable feature representation, while top layers of the network are task-specific for on-client personalization. Our proposed algorithm naturally resolves the statistical heterogeneity problem in federated networks. We are, to the best of knowledge, the first to provide both privacy and utility guarantees for such a proposed federated algorithm. The convergences are proved for the cases with Lipschitz smooth objective functions under the non-convex, convex, and strongly convex settings. Empirical experiment results on different datasets have been conducted to demonstrate the effectiveness of the proposed algorithm and verify the implications of the theoretical findings.

==> append_conv.tex <==
\section{Appendix}
In this appendix, we provide the details on the convergence proofs for the proposed \texttt{DPFedMTL} method. 

\subsection{Space Decomposition}
In this section, we describe how to decompose parameter space $\V$ into the composition of subspaces in order to analyze the convergence of our \texttt{DPFedMTL} methods. Due to the structure of our networks by splitting parameters into shared layers and client-specific layers, it is an essential problem of how to describe the splitting naturally. We achieve this goal by construct whole parameter space $\V$ by interpolating parameters of local clients to a high-dimensional space. A global optimization problem formulated in this high dimensional space is solved by subspace decomposition methods from the numerical analysis field \cite{chen2020randomized}. Firstly, we present transformation between local parameters $v_i$ of client $i$ and global parameters $w$ by restriction and interpolation operators defined in Definition~\ref{def:res_pro_operators}.

Let $w$ be a global parameter, i.e., $w = \begin{bmatrix} w_1 & w_2 & \cdots & w_{M+1} \end{bmatrix}^{\intercal} \in \V$, then 
$$
R_i w = \begin{bmatrix} w_i \\ \sqrt{1/M} w_{M+1} \end{bmatrix}, ~ 
I_i R_i w = \begin{bmatrix} 0 & \cdots & w_i & \cdots & \frac{1}{M} w_{M+1} \end{bmatrix}^{\intercal},
$$
where $w_i$ represents client-specific parameter and $w_{M+1}$ represents shared-layer parameter. 

Let $v_i$ be a local parameter embedded in whole space, i.e., $v_i = 
\begin{bmatrix} 0 & \cdots &  w_i  & \cdots & w_{M+1,i} \end{bmatrix}^{\intercal} \in \V$, and
$$
R_i v_i = \begin{bmatrix} w_i \\ \sqrt{1/M} w_{M+1,i} \end{bmatrix}, ~
I_i R_i v_i = \begin{bmatrix} 0 &  \cdots & w_i & \cdots & \frac{1}{M} w_{M+1,i} \end{bmatrix}^{\intercal}.
$$
where $w_i$ represents client-specific parameter and $w_{M+1,i}$ represents shared-layer parameter. 

The virtual global parameter is defined by an ensemble of local parameters
$
\bar{w} = \sum_{i \in [M]} I_i R_i v_i.
$
In Algorithm \ref{alg:DPFedMTL}, global parameter $w$ is updated by virtual global parameter every $H$ epochs by synchronization. 

Denote $\partial_i f(w) = \partial_{w_i} f(w)$ be partial derivative of function $f$ with respect to $i$-th component of $w$. 
With these two operators, we can rewrite the global objective function as follows:
\begin{equation}\label{eqn:obj_global_2}
f(w) 
= \frac{1}{M} \sum_{i=1}^M f_i( R_i w),
\end{equation}
where $f_i$ is local objective function. 
The update formula is $w^{t+1} = w^t - \eta^t g_i^t, $
where 
\begin{itemize}
\item Gradient at iteration $t$ when client $i$ is chosen. 
$$
g_i^t = \langle \partial_{i} f(w^t) , e_i \rangle + \frac{1}{M} \langle \partial_{M+1} f(w^t) , e_{M+1} \rangle 
$$
\item Perturbed gradient at iteration $t$ when client $i$ is chosen. 
$$
\tilde{g}_i^t = \langle \partial_{i} f(w^t) , e_i \rangle + \frac{1}{M} \langle \partial_{M+1} f(w^t) + n_{M+1}, e_{M+1} \rangle 
$$
\item 
Accumulation of $\tilde{g}_i^ t$ over subset $\I_t$. 
$$
g^t = \sum_{i \in \mathcal{I}_t} \tilde{g}_i^t. 
$$
\end{itemize}
Synchronization is given by 
$$ \bar{w}^{t} = \sum_{i=1}^M I_i R_i v_i^t,  $$
where $v_i^t  = \langle w_i, e_i \rangle + \langle w_{M+1, i}, e_{M+1} \rangle $
 is parameter of local client $i$.

%--------------------------------------------------------------------------------------------------------------------
%			Stable Decomposition
%----------------------------------------------------------------------------------------------------------------------
%\begin{lemma} Projection $\{ u_i\}_{i \in [M]}$ of $w$ to subspace $\V_i$ defined 
%$$
%u_i = I_i R_i w
%$$
%forms a stable decomposition of global parameter $w$, i.e. 
%$$
%\sum_{i \in [M]} \| u_i \|^2 \leq \| w \|^2. 
%$$
%\end{lemma}

We show a projection of global parameter $w$ to subspace $\V_i$ via restriction and interpolation operators form a stable decomposition of $w$. 

% \noindent\textbf{Proof of Lemma \ref{lem:s_decomp}.}
\subsubsection{Proof of Lemma \ref{lem:s_decomp}.}
\begin{proof}
By definition of restriction and interpolation operators in Definition~\ref{def:res_pro_operators}, 
$$
u_i = I_i R_i w = \begin{bmatrix} 0 & \cdots & w_i & \cdots & \frac{1}{M} w_{M+1} \end{bmatrix}^{\intercal}. $$
Then 
$$
\| u_i \|^2 = \|w_i \|^2 + (1/M)^2 \| w_{M+1}\|^2. 
$$
Summing over index $i$, 
\begin{eqnarray*}
\sum_{i=1}^M \|u_i\|^2 &= &\sum_{i=1}^M \left( \|w_i\|^2 + (1/M)^2  \| w_{M+1} \|^2 \right) \\
& \leq & \sum_{i=1}^{M+1} \|w_i \|^2  =   \|w \|^2. 
\end{eqnarray*}
\end{proof}


\subsection{Sufficient Decay}
%--------------------------------------------------------------------------------------------------------------------
%			Sufficient Decay
%----------------------------------------------------------------------------------------------------------------------

\begin{lemma} 
\label{lem:upper_inner}
Suppose the size of selected subset equals $1$, i.e. $K =1$ in Algorithm~\ref{alg:DPFedMTL} and sampling probability $\alpha_i = \frac{1}{M}$. Local update at step $t$ of selected client $i$ on local parameter $v_i^t$ is 
$$
\tilde{g}_i^t = 
\partial_{i} f_i (R_i v_i^t) + \sqrt{\frac{1}{M}} \partial_{M+1} f_i (R_i v_i^t) 
$$ 
and global update at virtual average $w^t$ is 
$$
\nabla f(\bar{w}^t) = \sum_{i=1}^M I_i \tilde{g}_i^t.
$$
There is a lower bound of inner product of local update and global update, i.e., 
\begin{eqnarray*}
 \E_{i, n} \left[ \langle \nabla f(\bar{w}^t), g^t \rangle \right]
& \geq & \frac{1}{M}   \| \nabla f(\bar{w}^t) \|^2 \\
& & - \frac{1}{2M}  \left[  \sum_{i=1}^M L_i^2 \|R_i \bar{w}^t - R_i v_i^t \|^2 \right],
\end{eqnarray*}
where $\bar{w}^t = \sum_{i \in [M]} I_i R_i v_i^t$ is virtual global parameter at step $t$. 
\end{lemma}


\begin{proof}
Let sample size $K = 1,$ i.e. $| \I_t | = 1$ and $\bar{w}^t = \sum_{i \in [M]} I_i R_i v_i^t$ 
be virtual average parameter at step $t$.
\begin{eqnarray*}
 && - \E_{i,n} \left[ \langle \nabla f(\bar{w}^t), g^t \rangle \right] \\
 &=&  -  \left[ \langle \nabla f(\bar{w}^t), \E_{i,n} [g^t] \rangle \right] \\
 &=& -  \sum_{i \in [M]}  \frac{1}{M} \left[ \langle \nabla f(\bar{w}^t), \E_n \tilde{g}_i^t \rangle \right] \\
 &=& -  \sum_{i \in [M]}  \frac{1}{M} \left[ \langle \nabla f(\bar{w}^t), g_i^t \rangle \right] \\
 &=&  - \frac{1}{M} \sum_{i \in [M]}  \langle \partial_{i} f_i(R_i \bar{w}^t), \partial_{i} f_i(R_i v_i^t) \rangle  \\
&&   - \frac{1}{M^2} \sum_{i \in [M]}  \langle \partial_{M+1} f_i(R_i \bar{w}^t), \partial_{M+1} f_i(R_i v_i^t) \rangle 
\end{eqnarray*}
The third equation is true since $\E_n [n_{M+1}] = 0$ and $\E_n{\tilde{g}_i^t} = g_i^t$.  
Furthermore, 
\begin{eqnarray*}
&&  -  \langle \partial_{i} f_i (R_i \bar{w}^t), \partial_{i} f_i (R_i v_i^t) \rangle \\
 &\leq & - \frac{1}{2} \| \partial_{i} f_i (R_i \bar{w}^t) \|^2 - \frac{1}{2} \| \partial_{i} f_i (R_i v_i^t) \|^2  \\
&&  + \frac{1}{2} \| \partial_{i} f_i(R_i \bar{w}^t) - \partial_{i} f_i(R_i v_i^t) \|^2 
\end{eqnarray*}
and 
\begin{eqnarray*}
&& -  \langle \partial_{M+1} f_i (R_i \bar{w}^t), \partial_{M+1} f_i (R_i v_i^t) \rangle \\
& \leq & - \frac{1}{2} \| \partial_{M+1} f_i (R_i \bar{w}^t) \|^2  - \frac{1}{2} \| \partial_{M+1} f_i (R_i v_i^t) \|^2 \\
& &+ \frac{1}{2}   \| \partial_{M+1} f_i(R_i \bar{w}^t) - \partial_{M+1} f_i(R_i v_i^t) \|^2 
\end{eqnarray*}

Consider full gradient of $f_i$ on $\bar{w}^t$. 
$$
\nabla \left( f_i(R_i \bar{w}^t) \right) = R_i^{\intercal} \nabla f_i(R_i \bar{w}^t) = \begin{bmatrix} \partial_i f_i(R_i \bar{w}^t) \\ \sqrt{1/M} \partial_{M+1} f_i(R_i \bar{w}^t) \end{bmatrix}
$$

The last term of both can be bounded by Local Lipschitz condition, i.e,
\begin{eqnarray*}
&& \frac{1}{2} \| \partial_{i} f_i (R_i \bar{w}^t) - \partial_{i} f_i (R_i v_i^t) \|^2 \\
&& + \frac{1}{2M} \| \partial_{M+1} f_i (R_i \bar{w}^t)  - \partial_{M+1} f_i (R_i v_i^t) \|^2  \\
& = & \frac{1}{2} \| \nabla f_i(R_i \bar{w}^t) - \nabla f_i(R_i v_i^t) \|^2 \\ 
& \leq & \frac{1}{2} L_i^2 \| R_i \bar{w}^t - R_i v_i^t \|^2  
\end{eqnarray*}

Thus 
\begin{eqnarray*}
- \E_{i, n} \left[ \langle \nabla f(\bar{w}^t), g^t \rangle \right]
%&\leq& - \frac{1}{2M} \sum_{i \in [M]} \left( \| \partial_i f_i (R_i w^t) \|^2 + \| \partial_i f_i (R_i v_i^t) \|^2 \right) \\
%&& - \frac{1}{2M^2} \left( \| \partial_{M+1} f_i (R_i w^t) \|^2 + \| \partial_{M+1} f_i (R_i v_i^t) \|^2 \right) \\
%&& + \frac{1}{2M} \sum_{i \in [M]} L_i^2 \| R_i w^t - R_i v_i^t \|^2 \\
%& \leq &- \frac{1}{2M} \left[   \| \nabla f(w^t) \|^2 +   \sum_{i \in [M]} \| \partial_{i} f_i (v_i^t) \|^2 \right] \\
%& & + \frac{1}{2M} \left[   \sum_{i=1}^M L_i^2  \|R_i w^t - v_i^t \|^2 \right]
& \leq &- \frac{1}{M}   \| \nabla f(\bar{w}^t) \|^2 \\
& & + \frac{1}{2M} \left[   \sum_{i=1}^M L_i^2  \|R_i w^t - R_i v_i^t \|^2 \right].
\end{eqnarray*}

\end{proof}


\begin{lemma} 
\label{lem:upper_2norm}
By same assumptions in Lemma \ref{lem:upper_inner} and Bounded Gradient Diversity Assumption, there is an upper bound of expectation of norm of update $g^t$, i.e., 
$$
\E_{i, n} [\| g^t\|^2] \leq \frac{1}{M} \left[ 
d_{M+1} \left( S \sigma \right)^2 + \lambda \| \nabla f(\bar{w}^t) \|^2 \right],
$$
where $i$ is index of the selected client and $n$ is Gaussian noise. 
\end{lemma}

\begin{proof}
For each selected client $i$, 
$$
\| g_i^t \|^2 = \| \partial_i f_i(R_i v_i^t) \|^2 + \frac{1}{M} \| \partial_{M+1} f_i(R_i v_i^t) + n_{M+1, i} \|^2. 
$$
Take expectation with respect to index of selected client $i$ and Gaussian noise $n$, we have 
\small{
\begin{eqnarray*}
\E_{i,n} \| g^t \|^2  &=& \frac{1}{M} \sum_{i \in [M]} \left[ \| \partial_{i} f_i(R_i v_i^t) \|^2  + \frac{1}{M} \| \partial_{M+1} f_i(R_i v_i^t) + n_{M+1,i} \|^2 \right] \\
%&=& \frac{1}{M} \left[ \sum_{i \in [M]} \| \partial_i f_i(R_i v_i^t) \|^2 + \frac{1}{M} \| \partial_{M+1} f_i(R_i v_i^t) \|^2 + (S \sigma)^2 \right] \\
&\leq & \frac{1}{M} \left[ \sum_{i \in [M]} \| \partial_{i} f_i(R_i v_i^t) \|^2 + \lambda \| \partial_{M+1} f_i(R_i \bar{w}^t) \|^2 \right] \\
&& + \frac{1}{M} d_{M+1}(S \sigma)^2,
\end{eqnarray*}}
where $\bar{w}^t = \sum_{i \in [M]} I_i R_i v_i^t$ and 
$$
\frac{M \sum_{i=1}^M \| \partial_{M+1} f_i(R_i v_i^t) \|^2}{\| \sum_{i=1}^M  \partial_{M+1} f_i(R_i \bar{w}^t) \|^2} \leq \lambda. 
$$
Specifically $\lambda > 1$ by convexity of $\ell_2$ norm, then we have 
$$
\E_{i, n} \| g^t\|^2 \leq \frac{1}{M} \left[ 
d_{M+1} \left( S \sigma \right)^2 + \lambda \| \nabla f(\bar{w}^t) \|^2 \right]. 
$$
\end{proof}

%--------------------------------------------------------------------------------------------------------------------
%
%			Synchronization influence 
%
%----------------------------------------------------------------------------------------------------------------------

\subsection{Synchronization Influence}

Since shared parameters are not synchronized every step, there would be a distance between local parameters $v_i^t$ and the virtual average parameters $\bar{w}^t$, which induces the difference between local updates and virtual global update. 
% If $H =1$, they attain the same value. 

\begin{lemma} 
\label{lem:syn_influ}
By the same assumptions in Lemma \ref{lem:upper_2norm} and Bounded Shared Gradient Assumption, 
suppose Algorithm \ref{alg:DPFedMTL} runs with a synchronization interval $H > 1$ and step-size $\eta$, there is an upper bound for the 
distance between local parameters $v_i^t$ and the virtual average $w^t$,
\begin{eqnarray*}
\frac{1}{M}  \sum_{i=1}^M \| R_i \bar{w}^t -R_i  v_i^t \|^2 &\leq& 4 \eta^2 H^2 (B^2 + d_{M+1} (S \sigma)^2). 
\end{eqnarray*}
\end{lemma}

\begin{proof}
Let $B$ be the uniform bound of partial gradient of shared layers, i.e. $ \| \partial_{M+1} f(\bar{w}^k)\| \leq B $ and $t_c$ be previous synchronized step, $t$ be current step, we have $\max_t |t - t_c | \leq H$. 
Follow L emma A.3 in \cite{mahdaviconvergence}, 
\begin{eqnarray*}
&& \frac{1}{M}  \E_{i,n}  \sum_{i=1}^M \| R_i \bar{w}^t - R_i v_i^t \|^2 \\
&=& 4 H \frac{1}{M} \sum_{k = t_c +1}^{t-1} \sum_{i=1}^M \eta^2 \| \partial_{M+1} f_i (R_i v_i^k) + n_{M+1, k} \|^2 \\ 
%&=& 4 H \frac{1}{M} \sum_{k=t_c +1}^{t-1} \sum_{i=1}^M \eta^2 \left( \| \partial_{M+1} f_i (R_i v_i^k) \|^2 + (S \sigma)^2 \right) \\
& \leq & 4 H \lambda \sum_{k=t_c +1}^{t-1} \eta^2 \| \sum_{i=1}^M \partial_{M+1} f( \bar{w}^k) \|^2  \\
&& + 4H \frac{1}{M} \sum_{k= t_c+1}^{t-1} \sum_{i=1}^M \eta^2 d_{M+1} (S \sigma)^2 \\
&\leq& 4 \eta^2 H^2 \left( \lambda B^2 + d_{M+1} (S \sigma)^2 \right)
\end{eqnarray*}
\end{proof}


% \noindent\textbf{Proof of Lemma \ref{lem:sd}.}
\subsubsection{Proof of Lemma \ref{lem:sd}.} 
$\\$
Combine Lemma \ref{lem:upper_inner}, \ref{lem:upper_2norm} and \ref{lem:syn_influ}, we have the following sufficient decay Lemma \ref{lem:sd} to describe how function value decays in two sequential steps in expectation. 
%\begin{lemma} [Sufficient Decay] 
%\label{lem:SD}
% Under the Lipschitz-continuous assumption of gradient function of global objective function $f$,  
%let $\{w^t\}$ be sequence generated by Algorithm \texttt{DPFedMTL} with Poisson sampling $\alpha_i=1/M$ and step-size $\eta = \frac{1}{2 \lambda L}$, we have 
%\begin{eqnarray*}
% \E_{i, n} \left[ f(w^{t+1}) \right] - f(w^t)  &\leq& 
% - \frac{1}{8 \lambda M L} \| \nabla f(w^t) \|^2  \\
% && + \frac{H^2} {4 \lambda^3 L}  B^2  \\
% && + \left( \frac{H^2}{4 \lambda^3 L} + \frac{1}{8 \lambda^2 M L} \right) d_{M+1} (S \sigma)^2. 
%\end{eqnarray*}
%where $L = \max_i L_i$, 
%$d_{M+1} $ is dimension of subspace $\V_{M+1}$, 
%$M$ is number of all clients, 
%$H$ is synchronization interval, 
%$B$ is upper bound for partial gradient on subspace $\V_{M+1}$, 
%$\lambda$ is the bound for gradient diversity, 
%$S$ is sensitivity of gradient operation, 
%and $S \sigma$ is magnitude of Gaussian noise $n$. 
%\label{lem:sd}
%\end{lemma}

\begin{proof}
Suppose client $i$ is selected at iteration $t$. 
$$
w^{t+1} = \bar{w}^t - \eta g^t = \bar{w}^t - \eta \tilde{g}_i^t 
$$

For each update $t$ we have 
$$
 f(w^{t+1}) - f(\bar{w}^t) \leq - \eta \langle \nabla f(\bar{w}^t), g^t \rangle + \frac{L}{2} \eta^2 \| g^t \|^2,
$$
where $L = \max_{i \in [M] } L_i. $

Take conditional expectation of random variable $w^{t+1}$ conditioned on $\bar{w}^t$ with respect to $i$ and Gaussian noise $n$ on both sides , we have 
$$
\E_{i,n} \left[ f(w^{t+1}) \right] - f(\bar{w}^t) \leq - \eta \E_{i,n} \langle  \nabla f(\bar{w}^t), g^t \rangle + \frac{L}{2} \eta^2 \E_{i,n} \| g^t \|^2 . 
$$

By previous Lemma \ref{lem:upper_inner} and \ref{lem:upper_2norm}, we have upper bounds of both $- \E_{i,n} \langle  \nabla f(\bar{w}^t), g^t \rangle$ and $\E_{i,n} \|g^t \|^2$.

\begin{eqnarray*}
- \E_{i, n} \left[ \langle \nabla f(\bar{w}^t), g^t \rangle \right]
& \leq &- \frac{1}{M} \left[   \| \nabla f(\bar{w}^t) \|^2  \right] \\
& & + \frac{1}{2M}  \left[  \sum_{i=1}^M L_i^2 \|R_i \bar{w}^t - R_i v_i^t \|^2 \right].
\end{eqnarray*}
And 
$$
\E_{i, n} [\| g^t\|^2] \leq \frac{1}{M} \left[ 
d_{M+1} \left( S \sigma \right)^2 +  \lambda  \| \nabla f(\bar{w}^t) \|^2 \right].
$$
Combine all, we get 
\begin{eqnarray*}
 \E_{i,n} \left[ f(w^{t+1}) \right] - f(w^t)  &\leq& \left( - \frac{\eta}{M} + \frac{\lambda L \eta^2}{2M} \right) \| \nabla f(\bar{w}^t) \|^2 \\
&& + \frac{L^2 \eta}{2M} \sum_{i=1}^M \|R_i w^t - R_i v_i^t \|^2 \\
&& + \frac{L \eta^2}{2M} d_{M+1} (S \sigma)^2 
\end{eqnarray*}

Notice that the third term is bounded by Lemma \ref{lem:syn_influ}. 
\begin{eqnarray*}
\frac{1}{M}  \sum_{i=1}^M \| R_i w^t -R_i  v_i^t \| &\leq& 4 \eta^2 H^2 (B^2 + d_{M+1} (S \sigma)^2). 
\end{eqnarray*}

Minimizing first term gives optimal step size as $\eta = \frac{1}{ \lambda L}$. Plug in previous equation, one can get 
\begin{eqnarray*}
 \E_{i, n} \left[ f(w^{t+1}) \right] - f(\bar{w}^t)  &\leq& 
 - \frac{1}{2 \lambda M L} \| \nabla f(\bar{w}^t) \|^2  \\
 && + \frac{H^2} {2 \lambda^2 }  B^2  \\
 && + \frac{1}{\lambda^2} \left( 2H^2 + \frac{1}{2ML} \right) d_{M+1} (S \sigma)^2. 
\end{eqnarray*}
\end{proof}


%---------------------------------------------------------------------------------------------
% Convergence for Nonconvex
%---------------------------------------------------------------------------------------------
% \noindent\textbf{Proof for Theorem~\ref{thm:nonconvexity}.}
\subsection{Proof for Theorem~\ref{thm:nonconvexity}.}
By the previous property of Sufficient Decay (Lemma \ref{lem:SD}), the convergence under Local Lipschitz Continuity and Global Non-convexity are proved as Theorem~\ref{thm:nonconvexity}. 

\begin{proof}
Recall sufficient decay conclusion in Lemma \ref{lem:SD}, 
\begin{eqnarray*}
 \E_{i, n} \left[ f(w^{t+1}) \right] - f(\bar{w}^t)  &\leq& 
 - \frac{1}{2 \lambda M L} \| \nabla f(\bar{w}^t) \|^2  \\
 && + \frac{H^2} {2 \lambda^2 }  B^2  \\
 && + \frac{1}{\lambda^2} \left( 2H^2 + \frac{1}{2ML} \right) d_{M+1} (S \sigma)^2. 
\end{eqnarray*}


Take full expectation, 
\begin{eqnarray*}
 \E \left[ f(w^{t+1}) \right] - \E f(\bar{w}^t)  &\leq& 
 - \frac{1}{2 \lambda M L} \E \| \nabla  f(\bar{w}^t) \|^2  \\
 && + \frac{H^2} {2 \lambda^2 }  B^2  \\
 && + \frac{1}{\lambda^2} \left( 2H^2 + \frac{1}{2ML} \right) d_{M+1} (S \sigma)^2. 
\end{eqnarray*}


Summing over $t$, 
\begin{eqnarray*}
f^* - f(w^0) &\leq &   \E[f(w^{T+1})] - f(w^0)  \\
& \leq &  - \frac{1}{2 \lambda M L} \E \sum_{t=0}^T \| \nabla f(\bar{w}^t) \|^2  \\
 && + \frac{H^2} {2 \lambda^2}  B^2 T  \\
 && + \frac{1}{\lambda^2} \left( 2 H^2 + \frac{1}{2 M L} \right) d_{M+1} (S \sigma)^2 T. 
\end{eqnarray*}

By rearranging terms and dividing $T$, we have the previous results. 
\end{proof}

%---------------------------------------------------------------------------------------------
%			Convergence for Convex and Lipschitz Continuous 
%---------------------------------------------------------------------------------------------
% \noindent\textbf{Proof for Theorem~\ref{thm:convexity}.}
\subsection{Proof for Theorem~\ref{thm:convexity}.}
By the previous property of Sufficient Decay (Lemma \ref{lem:SD}), we present details of convergence analysis under Local Lipschitz Continuity and Global Convexity for Theorem~\ref{thm:convexity}.

\begin{proof}
By Lemma \ref{lem:SD} and assumption of Bounded level set and denote 
$$\alpha^2 = 2 \lambda M L R_0^2 \left( \frac{H}{2 \lambda^2} B^2 + \frac{1}{\lambda^2} \left( 2H^2 + \frac{1}{2ML} \right) 
d_{M+1} (S \sigma)^2 \right) $$
\begin{eqnarray*}
\E[f(w^{t+1})] - f(w^t) &\leq&  - \frac{1}{2 \lambda M L} \left( \| \nabla f(w^t) \|^2 -  \frac{\alpha^2}{R_0^2} \right)  \\
				%&\leq& - \frac{1}{8 \lambda M L} \left( \frac{1}{R_0^2} \left( f(w^t) - f^* \right)^2 -\frac{\alpha^2}{R_0^2} \right) \\
				&=& - \frac{1}{2 \lambda M L R_0^2}\left(  \left( f(w^t) -f^* \right)^2 - \alpha^2 \right) \\
\end{eqnarray*}
Denote  $d^{t} = f(w^t) - f^*.$
Then 
\begin{eqnarray*}
\E d^{t+1} - d^t &\leq& -\frac{1}{2 \lambda ML  R_0^2} \left( (d^t)^2 - \alpha^2 \right) \\
\left( \E d^{t+1} - \alpha \right) - \left( d^t - \alpha \right) & \leq& - \frac{1}{2 \lambda M L  R_0^2} \left( (d^t)^2 - \alpha^2 \right) \\
\end{eqnarray*}
Since $\E d^{t+1} \leq d^t$ and $\E d^{t+1} - \alpha \leq d^t + \alpha, $
\begin{eqnarray*}
 \frac{1}{d^t - \alpha} - \frac{1}{\E d^{t+1} - \alpha} 
% \frac{\left( \E d^{t+1} - \alpha \right) - \left( d^t - \alpha \right)}{ \left(\E d^t - \alpha \right) \left( \E d^{t+1} -  \alpha \right) }  \\
%& \leq& \frac{\left( \E d^{t+1} - \alpha \right) - \left( d^t - \alpha \right)}{ \left(d^t - \alpha \right) \left( d^t + \alpha \right) } \\
 &\leq&  - \frac{1}{2 \lambda M L R_0^2} 
\end{eqnarray*}

Taking full expectation on both sides, as long as $\alpha < \E d^{t+1} < d^0, $
$$
\frac{1}{\E d^{t+1} - \alpha} - \frac{1}{\E d^t - \alpha} \geq \frac{1}{2 \lambda ML  R_0^2}. 
$$
Then 
$$
\frac{1}{E d^{t+1} - \alpha} \geq \frac{1}{d^0 - \alpha} + \frac{t+1}{2 \lambda M L  R_0^2}. 
$$
\end{proof}

%---------------------------------------------------------------------------------------------
%Convergence for Strongly Convex and Lipschitz Continuous 
%---------------------------------------------------------------------------------------------
% \noindent\textbf{Proof for Theorem~\ref{thm:strong_convexity}.}
\subsection{Proof for Theorem~\ref{thm:strong_convexity}.}
By the previous property of Sufficient Decay (Lemma \ref{lem:SD}), the convergence analysis under Local Lipschitz Continuity and Global Strongly Convexity for Theorem~\ref{thm:strong_convexity} are shown as the following. 
\begin{proof}
By Strong Convexity Assumption, we can prove  
$$
f(\bar{w}^t) - f^* \leq \frac{1}{2c} \| \nabla f(\bar{w}^t) \|_2^2. 
$$
Let
 $$\beta = \frac{\lambda ML}{c} \left( \frac{H^2}{2 \lambda^2} B^2 + \frac{1}{\lambda^2} \left( 2H^2 + \frac{1}{2ML} \right) 
d_{M+1} (S \sigma)^2 \right)$$. 
Combined with Lemma \ref{lem:SD}, we have 
$$
\E[f(w^{t+1})] - f(\bar{w}^t) \leq - \frac{c}{ \lambda M L} \left( f(\bar{w}^t) - f^* - \beta \right) . 
$$
Taking full expectation on both sides, we have 
\begin{eqnarray*}
\E[f(w^{t+1})] - f^*  &- & \beta  \\
& \leq &  \left(1 - \frac{c}{ \lambda M L} \right) \left(\E[f(\bar{w}^t)] - f^* - \beta \right).
\end{eqnarray*}
Then we have linear convergence of Algorithm \texttt{DPFedMTL}. 
\begin{eqnarray*}
\E[f(w^{T+1})] - f^* &-& \beta  \\
&  \leq & \left(1 - \frac{c}{ \lambda M L} \right)^{T+1} \left(f(w^0) - f^*  - \beta \right).
\end{eqnarray*}

\end{proof}
\newpage 

